GLASS: Global to Local Attention for Scene-Text Spotting

In recent years, the dominant paradigm for text spotting is to combine the tasks of text detection and recognition into a single end-to-end framework. Under this paradigm, both tasks are accomplished by operating over a shared global feature map extracted from the input image. Among the main challenges that end-to-end approaches face is the performance degradation when recognizing text across scale variations (smaller or larger text), and arbitrary word rotation angles. In this work, we address these challenges by proposing a novel global-to-local attention mechanism for text spotting, termed GLASS, that fuses together global and local features. The global features are extracted from the shared backbone, preserving contextual information from the entire image, while the local features are computed individually on resized, high-resolution rotated word crops. The information extracted from the local crops alleviates much of the inherent difficulties with scale and word rotation. We show a performance analysis across scales and angles, highlighting improvement over scale and angle extremities. In addition, we introduce an orientation-aware loss term supervising the detection task, and show its contribution to both detection and recognition performance across all angles. Finally, we show that GLASS is general by incorporating it into other leading text spotting architectures, improving their text spotting performance. Our method achieves state-of-the-art results on multiple benchmarks, including the newly released TextOCR.

==> chapters/eccv_plan.tex <==
\section{Planning for ECCV}

\subsection{Main Drawbacks}

Missing experiments and figures:
\begin{enumerate}
    \item TextOCR - without sin2 and with sin2, need to show impact on the detection - IN PROGRESS
    \item Angle on ICDAR13 Rot, need to show with and without sin2 - DONE
    \item A cherry pick renewed figure 4 - DONE
    \item A fail-case analysis figure - DONE in Supp.
    \item Add number of parameters in the performance comparison
    \item Adding a figure that shows that you need context for reading text - No time, this needs significant more work to prove the case. We'll need attention maps and show highlights
    \item Add/edit existing figure to showcase where the sin2 loss comes into play (comment from Inbal) 
    \item Add the rotated sine loss to Figure.2 - Done
\end{enumerate}

Benefits of sin2 loss
\begin{enumerate}
    \item Decouples the recognition task from the detection
    \item Pi-periodic, allows more consistent angle regression and performance
    \item Differentiable loss function
    \item Improves detection performance
    \item Contributes to overall E2E performance
\end{enumerate}


Supplementary additional materials
\begin{enumerate}
    \item Discuss how the sin2 loss benefits the anchors
    \item additional computational discussion, including parameters
    \item complementary detection ablation study for table 3 
\end{enumerate}

How to improve the text:
\begin{enumerate}
    \item Not clear whether improvement comes from the additional compute and params or from the novelty of the idea
    \item Lacking qualitative analysis of the results
    \item We are not educating the reader on new capabilities
    \item We did not show numbers with the cascaded system as ablation
    \item We do not have a discussion that connects between cascaded/e2e and what's in between
    \item Sine square loss can be better explained as a contribution
    \item We can draw ideas from what is wrong with text spotting. We need to provide more value to the reader
    % \item Rotated IC13 can be used to better leverage the sine-square loss
    \item The first contribution is too much. We should consider to make it simpler.
    \item We do not split the performance across different object sizes.
\end{enumerate}

\subsection{Tasks}
\begin{enumerate}
    \item Obtain results on TextOCR by approaching the organizers with our results.
    \item Overwhelming tables, need to fix columns and rows in all the ablation studies to make perfect sense and easier to read.
\end{enumerate}

\subsection{Analysis and Experiments}
\begin{enumerate}
    \item Roi - Format towards ECCV, and start working on the main body of text - DONE
    \item Roi - Fix the ablation study tables according to Manmatha's suggestions
    \item Roi - Move to a global/local terminology across the paper (instead of ROI/Crop).
    \item Roi + Shahar - Rewrite contributions:
    \begin{enumerate}
      \item We explore the relations between global and local contexts for scene text e2e and show that…
      \item We present an attention mechanism for cross-context fusion
      \item SoTA by a large margin for shlompi03, shlompi 15 and shlompi-21 rotated
      \end{enumerate}
      \item Shahar - Evaluate on Rotated IC13
    \item Shahar - Compare report on TotalText and ICDAR15, w/ and w/o HAIFA
    \item Shahar - Think on better scoping of the Sine Square loss
    \item Amir - Analysis of performance vs. crop size
    \item Shahar - output a evaluation dataframe of the predictions
    \item Amir - run a demo endpoint of HAIFA, and invoke "compare-two-runs" on it.
\end{enumerate}

==> tables/icdar13.tex <==
\begin{table}[t]
   \caption{\textbf{Results on Rotated ICDAR 2013 dataset.} F-measure of detection and end-to-end (E2E) recognition, under different rotation angles.}
\centering
\begin{tabular}{l|cccc|cccc|cccc}
\multirow{3}{*}{Method}  & \multicolumn{4}{c|}{$0$} & \multicolumn{4}{c|}{$45^{\circ}$} & \multicolumn{4}{c}{$60^{\circ}$} \\ 
\cmidrule(l){2-13} 
& \multicolumn{3}{c|}{Detection} & \multicolumn{1}{c|}{E2E}  & \multicolumn{3}{c|}{Detection} & \multicolumn{1}{c|}{E2E} 
& \multicolumn{3}{c|}{Detection} & \multicolumn{1}{c}{E2E}        \\   
& R & P & H  & H & R & P & H  & H & R & P & H & H\\
\hline
CharNet~\cite{liu2018char} & 81.7 & 82.3 & 82.0  &61.4 & 56.6 & 57.8 &57.2     & 33.9  &53.3 &65.5    & 58.8        & 9.3       \\
MTSv2~\cite{lyu2018mask}    & 85.3 & 89.9 & 87.5 &80.3 &   59.9   & 64.8 &  62.2& 54.2      & 61.2 & 70.5 &65.5   & 56.6    \\
MTSv3 \cite{liao2020spotterV3} & 84.4 &  90.5 &   87.4   & 80.2 &   77.9 & \textbf{91.6 }       & 84.2   & 76.1 &    79.4     & \textbf{90.7} & 84.7 &  76.6      \\
 \hline
\textbf{Ours + $L_1$ loss}      & {85.2} & \textbf{91.5} & {88.2}    & {82.2} & \textbf{80.9} & 91.4 & \textbf{85.8} & {79.4} &{ 78.8} & 89.2 & {83.7} &\textbf{77.4} \\
\textbf{Ours + $\sin^2$ loss}      & \textbf{88.3} & {91.3} & \textbf{89.8}    & \textbf{84.1} & {80.2} & 90.1 & {84.9} & \textbf{79.9} &\textbf{83.1} & 87.7 &\textbf{85.3} & { 77.0}
\end{tabular}
\label{table:rot_ic13}
\end{table}

==> tables/results_detection.tex <==
\begin{table}[t]
\small
\begin{tabular}{l|ccc|ccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c|}{Total-Text} & \multicolumn{3}{c}{ICDAR15} \\ \cline{2-7} 
\multicolumn{1}{c|}{}                        & R      & P      & H      & R         & P        & H        \\ \hline
CRAFT~\cite{baek2019craft}                   & 79.9   & 87.6   & 83.6   & 84.3    & 89.8   & 86.9     \\
DB~\cite{liao2020db}                         & 82.5   & 87.1   & 84.7   & 83.2    & \underline{91.8}   & 87.3     \\
MTS~\cite{lyu2018spotter}       & 82.4   & 88.3   & 85.2   & 87.3    & 88.6   & 87.0     \\
TFN-R50~\cite{ye2020textfusenet}     & 83.2   & 87.5   & 85.3   & \underline{88.9}    & 91.3   & \underline{90.1}     \\
TFN-R101~\cite{ye2020textfusenet}    & 85.3   & 89.0   & 87.1   & \textbf{89.7}    & \textbf{94.7}     & \textbf{92.1}     \\ 
ABCNet v2~\cite{liu2021abcnetV2}             & 84.1   & \underline{90.2}   & 87.0   & 86.0    & 90.4   & 88.1    \\ 
CRAFTS~\cite{baek2020crafts}                 & \underline{85.4}   & 89.5   & 87.4   & 85.3    & 89.0   & 87.1  \\
ABPN~\cite{zhang2021adaptive}                & 84.2  & \textbf{90.7}  & \underline{87.9}  & - & - & - \\ \hline
\textbf{Ours}       & \textbf{87.6}   &   \underline{90.2}     &  \textbf{ 88.9}               &        83.3   & 90.4         &   86.7
\\ \hline
\end{tabular}
\caption{Detection results on Total-Text and ICDAR15. R, P, and H refer to recall, precision and H-mean.}
\label{tab:res_detection}
\end{table}

==> tables/results_icdar.tex <==

\begin{table*}[t]
\small
\centering
\begin{tabular}{lcccccc}
\multirow{2}{*}{Method}  & \multicolumn{3}{c}{Word Spotting} & \multicolumn{3}{c}{End-to-end recognition} \\ \cline{2-4}  \cline{5-7} 
                         & S         & W         & G         & S            & W           & G            \\ \hline
                        
TextDragon~\cite{feng2019textdragon}   &     86.2      &    81.6       &     68.0       &         82.5         &   78.3   & 65.2         \\
ABCNet v2~\cite{liu2021abcnetV2}   &     -      &    -       &     -       &         82.7         &   78.5   & 73.0         \\
MTSv3*  (S-1440)~\cite{liao2020spotterV3}     & 83.1      & 79.1      & 75.1       & 83.3         & 78.1        & 74.2                 \\
Text Perceptron  (L-2000)~\cite{qiao2020text}           & 84.1        & 79.4        & 67.9  & 80.5      & 76.6     & 65.1               \\


CRAFTS (2560x1440)~\cite{baek2020crafts}          & -         & -         & -          & 83.1         & \textbf{82.1}        &     \underline{74.9}      \\
MANGO*$^\dagger$ (L-1800)~\cite{qiao2020mango}          & {85.2}      & 81.1      & 74.6      & \textbf{85.4}         & \underline{80.1}        & 73.9    \\
YAMTS* (1600x960)~\cite{krylov2021yamts}        & \textbf{86.8}      & \underline{82.4}      & \underline{76.7}       & \underline{85.3}         & 79.8        & 74.0            \\  \hline
% \multicolumn{1}{l}{Ours* (training w/o mask head) (S-1600)} &   84.5 %cfg.INFERENCE_TH_TEST = 0.1
% &       79.7  %cfg.INFERENCE_TH_TEST = 0.2 
% &    75.9&    73.9%cfg.MODEL.ROI_HEADS.NMS_THRESH_TEST = 0.1 cfg.INFERENCE_TH_TEST = 0.5
% &    85.2 %    cfg.MODEL.ROI_HEADS.NMS_THRESH_TEST = 0.5    cfg.INFERENCE_TH_TEST = 0.1 
% &     78.8  %    cfg.MODEL.ROI_HEADS.NMS_THRESH_TEST = 0.1    cfg.INFERENCE_TH_TEST = 0.4
% &      {74.75}& 73.0     \\ 
\multicolumn{1}{l}{\textbf{Ours* (L-1600)}} 
&   \textbf{86.8}
&      \textbf{ 82.5 }
&    \textbf{78.8}
&    {84.7}
&     \underline{80.1}
&    \textbf{76.3}
% \\
% \multicolumn{1}{l}{\textbf{Ours* - R101 (L-1600)}}
% &  ?? 
% &      ?? 
% &    ??
% &    ??
% &    ?? 
% &     ?? 

 \\
\hline
\end{tabular}

\caption{Results on ICDAR 2015 dataset. ‘S’, ‘W’ and ‘G’ mean recognition with strong, weak and
generic lexicon, respectively.  Prefix ‘L-’ and ‘S-’ represent that the input images  longer or shorter side is resized. * means that the method uses the specific lexicons from~\cite{liao2020spotterV3}. 
$^\dagger$ means that the method used IoU of 0.1 instead of 0.5.}
\label{tab:res_icdar}
\end{table*}

==> tables/results_icdar_temp.tex <==

\begin{table*}[!t]
\centering
% \begin{center}
\begin{tabular}{l cccc cccc} % \hspace*{} for Left-right shift of the entire table
\toprule

 &  \multicolumn{4}{c}{\textbf{NTU-RGB+D}} & \multicolumn{4}{c}{\textbf{Kinetics-250}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
\multicolumn{1}{l}{} & \multicolumn{2}{c}{{Few vs.\ Many}} & \multicolumn{2}{c}{{Many vs.\ Few}} & \multicolumn{2}{c}{{Few vs.\ Many}} & \multicolumn{2}{c}{{Many vs.\ Few}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
\textbf{Method} & \textit{Random} & \textit{Meaningful} & \textit{Random} & \textit{Meaningful} & \textit{Random} & \textit{Meaningful} & \textit{Random} & \textit{Meaningful} \\
\midrule	

Supervised         & \underline{0.86} & \underline{0.83} & 
 \underline{0.82} & \underline{0.90} &
 \underline{0.77} & 0.71 &
 \underline{0.63} & \underline{0.82}  \\
\midrule            
Rec. Loss                
& 0.50 & 0.54  
& 0.53 & 0.54  
& 0.45 & 0.46  
& 0.51 & 0.61  \\
OC-SVM                    
& 0.60 & 0.67 
& 0.60 & 0.69 
& 0.56 & 0.56 
& 0.52 & 0.47 \\ 
Liu \etal \cite{Liu_2018} 
& 0.57 & 0.64 
& 0.56 & 0.63 
& 0.55 & 0.60 
& 0.55 & 0.58 \\
Morais \etal \cite{Morais_2019_CVPR} & - & - & - & - 
& 0.57 & 0.59 
& 0.56 & 0.58 \\
Ours                      
& \textbf{0.73} & \textbf{0.82} 
& \textbf{0.72} & \textbf{0.85} 
& {\textbf{0.65}} & {\underline{\textbf{0.73}}}  
& {\textbf{0.62}} & {\textbf{0.74}} \\
\bottomrule
\end{tabular}
% \end{center}
\vspace{0.08cm}		
\caption{ {\bf Coarse-Grained Experiment Results:} Values represent area under the ROC curve (AUC). In bold are the results of the best performing \emph{unsupervised} method. Underlined is the best method of all. For all experiments $K=20$ clusters, see section~\ref{method:deep_clustering} for details. 
% For random choice, AUC=0.50.
It~should be noted that AUC=0.50 in case of random choice.
}
\vspace{-0.3cm}
\label{tables:results}
\end{table*}	

==> tables/results_totaltext.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{lcccccc}

\multirow{2}{*}
{Method}                                               & \multicolumn{2}{c}{Word Spotting}       &  \multicolumn{2}{c}{End-to-End} 
                                                                                              
\\ \cline{2-3}  \cline{4-5} 
                                                    & None                 & Full   & None                 & Full                          \\ \hline
TextDragon~\cite{feng2019textdragon}        & - & -        & 48.8                & 71.8           \\
ABCNet~\cite{liu2020abcnet}                                                         & 64.2                & 75.7        & - & -        \\

ABCNet v2~\cite{liu2021abcnetV2}                                                      &   70.4                   &    78.1       & - & -           \\
MTSv3 (S-1000)~\cite{liao2020spotterV3}          & - & -          & 71.2                 & {78.4}             \\
Text Perceptron  (L-2000)~\cite{qiao2020text}                   & 69.7                 & {78.3}        & - & -         \\
MANGO$^{\dagger}$ (L-1600)~\cite{qiao2020mango}                                & \underline{72.9}                 & \underline{83.6}     & 68.9$^\ddagger$	 & \underline{78.9}$^\ddagger$            \\
CRAFTS (L-1920)~\cite{baek2020crafts}            &- & -   &\textbf{78.7}        & -                    \\
YAMTS (1280x768)~\cite{krylov2021yamts}            & - & -                         & 71.1                 & {78.4}               \\ \hline
\textbf{Ours (S-1000)}         & \textbf{79.9} & \textbf{86.2} &  \underline{76.6}
&   \textbf{83.0} \\
\hline
\end{tabular}
\caption{Results on Total-Text validation. “None” refers to recognition without any lexicon.
“Full” lexicon contains all words in test set. 
$^\dagger$ means that the method uses IoU of 0.1 instead of 0.5. $^\ddagger$ represents results taken from the official method's source code.}
\label{tab:res_totaltext}
\end{table*}



% \begin{table}
% \centering
% \small
% \begin{tabular}{lcccc}
% \hline
% \multirow{2}{*}
% {Method}                                                     & \multicolumn{2}{c}{End-to-End} 
                                                                                              
% \\ \cline{2-3} 
%                                                     & None                 & Full                            \\ \hline
% TextDragon~\cite{feng2019textdragon}                & 48.8                & 71.8                \\
% ABCNet~\cite{liu2020abcnet}                                                         & 64.2                & 75.7                \\

% ABCNet v2~\cite{liu2021abcnetV2}                                                      &   70.4                   &    78.1                  \\
% Mask TextSpotter v3* (S-1000)~\cite{liao2020spotterV3}                    & 71.2                 & {78.4}             \\
% Text Perceptron  (L-2000)~\cite{qiao2020text}                   & 69.7                 & {78.3}             \\
% MANGO*$^\dagger$ (L-1600)~\cite{qiao2020mango}                                & 72.9                 & \textbf{83.6}                 \\
% CRAFTS (L-1920)~\cite{baek2020crafts}                                  & \textbf{78.7}        & -                 \\
% YAMTS* (1280x768)~\cite{krylov2021yamts}                                 & 71.1                 & {78.4}               \\ \hline
% \textbf{Ours* (S-1000)}                                                              & \underline{76.6}
% &   \underline{83.0} \\
% \hline
% \end{tabular}
% \caption{Results on Total-Text validation. “None” refers to recognition without any lexicon.
% “Full” lexicon contains all words in test set. * means that the method uses the specific lexicons from Liao et al. (2019). 
% $^\dagger$ means that the method uses IoU of 0.1 instead of 0.5.}
% \label{tab:res_totaltext}
% \end{table}

==> tables/textocr_results_test.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Results on the TextOCR test dataset.}  R, P, and H refer to recall, precision and H-mean. The results are lexicon-free. We report the result for Mask TextSpotter v3 from~\cite{singh2021textocr}, where it was trained also with TextOCR train data.} 
\label{tab:res_textocr_test}
\begin{tabular}{l|ccc||ccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c||}{Word Spotting}&   \multicolumn{3}{c}{End-to-End} \\ \cline{2-7} 
\multicolumn{1}{c|}{}                        & R      & P      & H      & R      & P      & H        \\ \hline
MTSv3~\cite{liao2020spotterV3} & -   & -   & -   & - & - & 50.8    \\ \hline
\textbf{Baseline}       &{46.3}   &   {77.5}     &  {58.0}               &    45.3    & 76.0 & 56.8
\\
\textbf{Ours}       & \textbf{60.3}   &   \textbf{84.5}     &  \textbf{70.4}      & \textbf{58.4}         &        \textbf{78.9} &        \textbf{67.1}
\\ \hline
\end{tabular}
\end{table}

